Coordinated Motion Planning: Reconfiguring a Swarm of Labeled Robots with Bounded Stretch

We present a number of breakthroughs for coordinated motion planning, in which the objective is to reconfigure a swarm of labeled convex objects by a combination of parallel, continuous, collision-free translations into a given target arrangement. Problems of this type can be traced back to the classic work of Schwartz and Sharir (1983), who gave a method for deciding the existence of a coordinated motion for a set of disks between obstacles; their approach is polynomial in the complexity of the obstacles, but exponential in the number of disks. Other previous work has largely focused on {\em sequential} schedules, in which one robot moves at a time. We provide constant-factor approximation algorithms for minimizing the execution time of a coordinated, {\em parallel} motion plan for a swarm of robots in the absence of obstacles, provided some amount of separability. Our algorithm achieves {\em constant stretch factor}: If all robots are at most $d$ units from their respective starting positions, the total duration of the overall schedule is $O(d)$. Extensions include unlabeled robots and different classes of robots. We also prove that finding a plan with minimal execution time is NP-hard, even for a grid arrangement without any stationary obstacles. On the other hand, we show that for densely packed disks that cannot be well separated, a stretch factor $\Omega(N^{1/4})$ may be required. On the positive side, we establish a stretch factor of $O(N^{1/2})$ even in this case.

==> 04-unlabeled-grid.tex <==
In this section we show how to extend our approach of Section~\ref{sec:constappr}
to %an $\mathcal{O}(1)$-approximation for
the \emph{unlabeled} and, more generally, the \emph{colored} variant of the
parallel robot motion-planning problem.  We formalize this problem variant by
using a coloring $c: \{ 1,\dots,n_1n_2 \} \rightarrow \{
1,\ldots,k \}$ for grouping the robots.
By populating unoccupied cells with robots carrying color $k+1$, we may assume that
each unit square in the environment $P$ is occupied.
The robots \emph{draw an image} $I = \big(I^1,\ldots,I^k\big)$, where $I^i$ is the set of cells occupied by a robot with color $i$. \textcolor{black}{We say that two images $I_s$ and $I_t$ are \emph{compatible} if in $I_s$ and $I_t$ the number of cells colored with color $i$ are equal for each color $i = 1,\dots,k$.}
By moving the robots, we want to transform a start image $I_s$ into a target image $I_t$, minimizing the makespan.

\begin{theorem}\label{thm:unlabeled}
There is an algorithm with running time $\mathcal{O}(k(n_1n_2)^{1.5} \log (n_1n_2) + dn_1n_2)$ that computes, given \textcolor{black}{compatible} start and target images $I_s,I_t$, 
an $\mathcal{O}(1)$-approximation of the optimal makespan $M$ and a corresponding sequence of transformation steps.
\end{theorem}

\begin{proof}
	We transform the input into an instance of the labeled variant such that an $\mathcal{O}(1)$-approximation for the labeled instance provides an $\mathcal{O}(1)$-approximation for the colored instance. 
	For each color $i$, we consider the two point sets $A^i,B^i \subset \mathbb{R}^2$, where $A^i$ contains the center points $a^i_v$ of all unit squares $v \in I^i_s$ and $B^i$ contains the center points $b^i_v$ of all $v \in I^i_t$.

	A {\em bottleneck matching} between $A^i$ and $B^i$ is a perfect matching between $A^i$ and $B^i$ minimizing the maximal distance.
	The cost of an optimal bottleneck matching between $A^i$ and $B^i$ is in $\mathcal{O}(M)$ because a transformation sequence induces a bottleneck matching on all color classes.
	Efrat et al.~\cite{efrat:geometry} show that the geometric bottleneck matching problem can be solved in $\mathcal{O}(|A+B|^{1.5} \log |A+B|)$ time.

	A set of $k$ bottleneck matchings between the sets $A^i$ and $B^i$ induces labeled start and target configurations $C_s,C_t$.
	Applying the algorithm from Section~\ref{sec:constappr} to these yields a sequence of transformation steps of length $\mathcal{O}(M)$.
\end{proof}



